A Systematic Review of Business Process Improvement: Achievements and Potentials in Combining Concepts from Operations Research and Business Process Management

Business Process Management and Operations Research are two research fields that both aim to enhance value creation in organizations. While Business Process Management has historically emphasized on providing precise models, Operations Research has focused on constructing tractable models and their solutions. This systematic literature review identifies and analyzes work that uses combined concepts from both disciplines. In particular, it analyzes how business process models have been conceptualized as mathematical models and which optimization techniques have been applied to these models. Results indicate a strong focus on resource allocation and scheduling problems. Current approaches often lack support of the stochastic nature of many problems, and do only sparsely use information from process models or from event logs, such as resource-related information or information from the data perspective.

==> chapters/02_foundations/02_00_BPM.tex <==
\subsection{Business Process Management}
%
\enquote{Business Process Management (BPM) is the art and science of overseeing how work is performed in an organization to ensure consistent outcomes and to take advantage of improvement opportunities} \citep{dumas_fundamentals_2018}.
As such, BPM is concerned with different levels of abstraction. \citet{weske_business_2019} has defined four levels of abstraction: Business goals and strategies, organizational business processes, operational business processes, and implemented business processes.
Operational business processes are specified by process models, while implemented business processes are formal business process models enriched with run-time data.
Therefore, operational and implemented business processes can be analyzed with formal techniques.
\\
Operational business process models can again be divided into imperative and declarative business process models.
Several business process modeling languages have been defined to specify imperative operational processes, such as the Business Process Modeling Notation (BPMN), UML activity diagrams, or Petri nets, or to specify declarative process models, such as Declare, or Guard-Stage-Milestones (GSM).
%

==> chapters/02_foundations/02_00_OR.tex <==
\subsection{Operations Research}
%
OR is a broad discipline.
In this work, we follow the short definition of  \citet{eiselt_operations_2022} that \enquote{operations research is concerned with quantitative (mathematical) models and their solution}.
\\
OR has a long history in resource planning and production planning, allocating resources to activities (jobs), and scheduling the execution of activities.
Exemplary, in the European Journal of Operations Research, the OR journal with the highest number of articles published, \enquote{scheduling} has been the most used keyword throughout the journal's 40 years of history, while it has been surpassed in the 2010-2016 period by the keyword \enquote{supply chain management} \citep{laengle_forty_2017}.
%
\subsubsection{Project Scheduling}
%
Projects in OR are related to business processes, as they have a defined start and end state, pursue a defined goal, and use a set of resources \citep{hillier_project_2002}.
Projects are typically represented as directed graphs, either in the activity-on-arrow notation or the activity-on-node notation.
The directed graph represents a precedence relationship: an activity may not be executed before its preceding activities have been completed.
Prescribing minimal or maximal time lag between to execution of a pair of activities can furthermore be been investigated under to term of generalized precedence relations (GPRs).
%
Project scheduling problems are commonly classified using the three-field notation $\alpha|\beta|\gamma$ in which $\alpha$ represents the resource characteristics, $\beta$ the activity characteristics, and $\gamma$ the optimality criterion.
%
Project scheduling problems that consider resources are known as Resource Constrained Project Scheduling Problems (RCPSPs).


\begin{comment}
\cite{Dumas2013}: The process performance measures are time, cost, quality and flexibility.


\\
\\
To the best of our knowledge, no approach has yet been undertaken to holistically review business process optimization methods throughout all business process life-cycle phases.

\end{comment}

==> chapters/02_foundations/02_foundations.tex <==
\section{Foundations}
\label{sec:foundations}
%
%
%
%
%
%
\input{chapters/02_foundations/02_00_BPM}
\input{chapters/02_foundations/02_00_OR}

==> chapters/04_results/04_00_overview.tex <==
Pavlos Delias
